A priori compression of convolutional neural networks for wave simulators

Convolutional neural networks are now seeing widespread use in a variety of fields, including image classification, facial and object recognition, medical imaging analysis, and many more. In addition, there are applications such as physics-informed simulators in which accurate forecasts in real time with a minimal lag are required. The present neural network designs include millions of parameters, which makes it difficult to install such complex models on devices that have limited memory. Compression techniques might be able to resolve these issues by decreasing the size of CNN models that are created by reducing the number of parameters that contribute to the complexity of the models. We propose a compressed tensor format of convolutional layer, a priori, before the training of the neural network. 3-way kernels or 2-way kernels in convolutional layers are replaced by one-way fiters. The overfitting phenomena will be reduced also. The time needed to make predictions or time required for training using the original Convolutional Neural Networks model would be cut significantly if there were fewer parameters to deal with. In this paper we present a method of a priori compressing convolutional neural networks for finite element (FE) predictions of physical data. Afterwards we validate our a priori compressed models on physical data from a FE model solving a 2D wave equation. We show that the proposed convolutinal compression technique achieves equivalent performance as classical convolutional layers with fewer trainable parameters and lower memory footprint.

==> Tables/testuf3.tex <==
\begin{table}[H]
\caption{Test error on full displacement}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{11.85} & \textcolor{red}{5.38} & \textcolor{red}{13.05} & \textcolor{red}{10.12} & \textcolor{red}{5.42} & \textcolor{red}{9.81} \\ \hline
Conv2D & \textcolor{blue}{0.67} & \textcolor{blue}{0.52} & \textcolor{blue}{0.52} & \textcolor{blue}{0.55} & \textcolor{red}{1.38} & \textcolor{blue}{0.54} \\ \hline
Conv2D t & \textcolor{red}{1.33} & \textcolor{red}{1.25} & \textcolor{red}{1.55} & \textcolor{red}{1.61} & \textcolor{red}{1.31} & \textcolor{red}{1.84} \\ \hline
Conv3D & \textcolor{red}{3.05} & \textbf{0.34} & \textcolor{blue}{0.44} & \textcolor{blue}{0.54} & \textcolor{blue}{0.35} & \textcolor{blue}{0.51} \\ \hline
Conv2.5D & \textcolor{blue}{0.54} & \textcolor{blue}{0.46} & \textcolor{blue}{0.56} & \textcolor{blue}{0.55} & \textcolor{blue}{0.44} & \textcolor{blue}{0.56} \\ \hline
Conv2.5Db & \textcolor{red}{1.09} & \textcolor{red}{0.81} & \textcolor{red}{0.81} & \textcolor{red}{0.76} & \textcolor{red}{0.69} & \textcolor{blue}{0.61} \\ \hline
\end{tabular}
\label{TestUF3}
\end{center}
\end{table}


==> Tables/testufz3.tex <==
\begin{table}[H]
\caption{Test error on displacement after zoom}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{11.85} & \textcolor{red}{5.38} & \textcolor{red}{13.05} & \textcolor{red}{10.12} & \textcolor{red}{5.42} & \textcolor{red}{9.81} \\ \hline
Conv2D & \textcolor{red}{0.67} & \textcolor{red}{0.52} & \textcolor{red}{0.52} & \textcolor{red}{0.55} & \textcolor{red}{1.38} & \textcolor{red}{0.54} \\ \hline
Conv2D t & \textcolor{red}{1.33} & \textcolor{red}{1.25} & \textcolor{red}{1.55} & \textcolor{red}{1.61} & \textcolor{red}{1.31} & \textcolor{red}{1.84} \\ \hline
Conv3D & \textcolor{red}{3.05} & \textcolor{red}{0.34} & \textcolor{red}{0.44} & \textcolor{red}{0.54} & \textcolor{red}{0.35} & \textcolor{red}{0.51} \\ \hline
Conv2.5D & \textcolor{red}{0.54} & \textcolor{red}{0.46} & \textcolor{red}{0.56} & \textcolor{red}{0.55} & \textcolor{red}{0.44} & \textcolor{red}{0.56} \\ \hline
Conv2.5Db & \textcolor{red}{1.09} & \textcolor{red}{0.81} & \textcolor{red}{0.81} & \textcolor{red}{0.76} & \textcolor{red}{0.69} & \textcolor{red}{0.61} \\ \hline
FC t Boundary & \textcolor{red}{5.92} & \textcolor{red}{3.03} & \textcolor{red}{7.77} & \textcolor{red}{7.83} & \textcolor{red}{4.11} & \textcolor{red}{6.18} \\ \hline
Conv1D Boundary & \textcolor{blue}{0.06} & \textbf{0.04} & \textcolor{blue}{0.06} & \textcolor{blue}{0.07} & \textcolor{blue}{0.08} & \textcolor{blue}{0.05} \\ \hline
Conv1D t Boundary & \textcolor{red}{0.41} & \textcolor{red}{0.44} & \textcolor{red}{0.42} & \textcolor{red}{0.55} & \textcolor{red}{0.65} & \textcolor{red}{0.53} \\ \hline
Conv2D Boundary & \textcolor{red}{0.11} & \textcolor{blue}{0.07} & \textcolor{red}{0.09} & \textcolor{red}{0.10} & \textcolor{blue}{0.08} & \textcolor{red}{0.11} \\ \hline
Conv1.5D Boundary & \textcolor{red}{0.12} & \textcolor{red}{0.11} & \textcolor{red}{0.10} & \textcolor{red}{0.11} & \textcolor{red}{0.11} & \textcolor{red}{0.11} \\ \hline
\end{tabular}
\label{TestUFZ3}
\end{center}
\end{table}


==> Tables/testvf3.tex <==
\begin{table}[H]
\caption{Test error on full velocity}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{5.06} & \textcolor{red}{1.86} & \textcolor{red}{5.10} & \textcolor{red}{4.81} & \textcolor{red}{2.44} & \textcolor{red}{4.81} \\ \hline
Conv2D & \textcolor{red}{2.21} & \textcolor{red}{2.15} & \textcolor{red}{2.25} & \textcolor{red}{2.14} & \textcolor{red}{2.64} & \textcolor{red}{2.18} \\ \hline
Conv2D t & \textcolor{blue}{0.63} & \textbf{0.61} & \textcolor{blue}{0.70} & \textcolor{blue}{0.76} & \textcolor{blue}{0.66} & \textcolor{blue}{0.82} \\ \hline
Conv3D & \textcolor{red}{138.39} & \textcolor{red}{2.00} & \textcolor{red}{2.08} & \textcolor{red}{2.14} & \textcolor{red}{2.05} & \textcolor{red}{2.13} \\ \hline
Conv2.5D & \textcolor{red}{2.18} & \textcolor{red}{2.09} & \textcolor{red}{2.12} & \textcolor{red}{2.09} & \textcolor{red}{2.09} & \textcolor{red}{2.12} \\ \hline
Conv2.5Db & \textcolor{red}{2.29} & \textcolor{red}{2.26} & \textcolor{red}{2.36} & \textcolor{red}{2.25} & \textcolor{red}{2.19} & \textcolor{red}{2.19} \\ \hline
\end{tabular}
\label{TestVF3}
\end{center}
\end{table}


==> Tables/testvfz3.tex <==
\begin{table}[H]
\caption{Test error on velocity after zoom}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{10.46} & \textcolor{red}{4.35} & \textcolor{red}{10.38} & \textcolor{red}{8.50} & \textcolor{red}{4.55} & \textcolor{red}{8.27} \\ \hline
Conv2D & \textcolor{red}{0.23} & \textcolor{red}{0.18} & \textcolor{red}{0.22} & \textcolor{red}{0.25} & \textcolor{red}{0.20} & \textcolor{red}{0.21} \\ \hline
Conv2D t & \textcolor{red}{0.90} & \textcolor{red}{0.75} & \textcolor{red}{0.77} & \textcolor{red}{0.96} & \textcolor{red}{0.87} & \textcolor{red}{1.14} \\ \hline
Conv3D & \textcolor{red}{1.75} & \textcolor{blue}{0.17} & \textcolor{red}{0.21} & \textcolor{red}{0.22} & \textcolor{red}{0.18} & \textcolor{red}{0.23} \\ \hline
Conv2.5D & \textcolor{red}{0.33} & \textcolor{red}{0.27} & \textcolor{red}{0.30} & \textcolor{red}{0.30} & \textcolor{red}{0.24} & \textcolor{red}{0.29} \\ \hline
Conv2.5Db & \textcolor{red}{0.41} & \textcolor{red}{0.41} & \textcolor{red}{0.44} & \textcolor{red}{0.40} & \textcolor{red}{0.39} & \textcolor{red}{0.38} \\ \hline
FC t Boundary & \textcolor{red}{6.42} & \textcolor{red}{3.39} & \textcolor{red}{7.64} & \textcolor{red}{7.30} & \textcolor{red}{3.74} & \textcolor{red}{6.33} \\ \hline
Conv1D Boundary & \textcolor{blue}{0.11} & \textbf{0.09} & \textcolor{blue}{0.11} & \textcolor{blue}{0.11} & \textcolor{blue}{0.11} & \textcolor{blue}{0.11} \\ \hline
Conv1D t Boundary & \textcolor{red}{0.48} & \textcolor{red}{0.48} & \textcolor{red}{0.46} & \textcolor{red}{0.58} & \textcolor{red}{0.73} & \textcolor{red}{0.56} \\ \hline
Conv2D Boundary & \textcolor{blue}{0.14} & \textcolor{blue}{0.11} & \textcolor{blue}{0.13} & \textcolor{blue}{0.14} & \textcolor{blue}{0.11} & \textcolor{blue}{0.14} \\ \hline
Conv1.5D Boundary & \textcolor{blue}{0.16} & \textcolor{blue}{0.14} & \textcolor{blue}{0.14} & \textcolor{blue}{0.16} & \textcolor{blue}{0.16} & \textcolor{blue}{0.15} \\ \hline
\end{tabular}
\label{TestVFZ3}
\end{center}
\end{table}


==> Tables/trainepoch2.tex <==
\begin{table}[H]
\caption{Average time of one epoch}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv2D & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv2D t & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv3D & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv2.5D & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv2.5Db & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
FC t Boundary & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv1D Boundary & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv1D t Boundary & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv2D Boundary & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
Conv1.5D Boundary & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} \\ \hline
\end{tabular}
\label{trainepoch2}
\end{center}
\end{table}


==> Tables/trainepoch3.tex <==
\begin{table}[H]
\caption{Average time of one epoch}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{0.47} & \textcolor{red}{0.51} & \textcolor{red}{0.51} & \textcolor{red}{0.50} & \textcolor{red}{0.52} & \textcolor{red}{0.51} \\ \hline
Conv2D & \textcolor{red}{0.66} & \textcolor{red}{0.67} & \textcolor{red}{0.63} & \textcolor{red}{0.45} & \textcolor{red}{0.48} & \textcolor{red}{0.53} \\ \hline
Conv2D t & \textcolor{blue}{0.37} & \textcolor{red}{0.41} & \textcolor{red}{0.65} & \textcolor{blue}{0.34} & \textcolor{red}{0.39} & \textcolor{red}{0.63} \\ \hline
Conv3D & \textcolor{blue}{0.33} & \textcolor{blue}{0.34} & \textcolor{red}{0.79} & \textcolor{blue}{0.27} & \textcolor{blue}{0.29} & \textcolor{red}{0.73} \\ \hline
Conv2.5D & \textcolor{red}{0.69} & \textcolor{red}{0.75} & \textcolor{red}{1.08} & \textcolor{red}{0.67} & \textcolor{red}{0.75} & \textcolor{red}{1.05} \\ \hline
Conv2.5Db & \textcolor{red}{1.09} & \textcolor{red}{1.20} & \textcolor{red}{1.67} & \textcolor{red}{1.06} & \textcolor{red}{1.07} & \textcolor{red}{1.52} \\ \hline
FC t Boundary & \textcolor{blue}{0.20} & \textcolor{blue}{0.21} & \textcolor{blue}{0.23} & \textbf{0.19} & \textcolor{blue}{0.21} & \textcolor{blue}{0.23} \\ \hline
Conv1D Boundary & \textcolor{blue}{0.35} & \textcolor{blue}{0.36} & \textcolor{red}{0.47} & \textcolor{blue}{0.28} & \textcolor{blue}{0.30} & \textcolor{red}{0.39} \\ \hline
Conv1D t Boundary & \textcolor{blue}{0.35} & \textcolor{blue}{0.36} & \textcolor{red}{0.51} & \textcolor{blue}{0.34} & \textcolor{blue}{0.35} & \textcolor{red}{0.51} \\ \hline
Conv2D Boundary & \textcolor{blue}{0.25} & \textcolor{blue}{0.23} & \textcolor{blue}{0.33} & \textcolor{blue}{0.19} & \textcolor{blue}{0.21} & \textcolor{blue}{0.28} \\ \hline
Conv1.5D Boundary & \textcolor{red}{0.69} & \textcolor{red}{0.73} & \textcolor{red}{1.06} & \textcolor{red}{0.65} & \textcolor{red}{0.69} & \textcolor{red}{1.02} \\ \hline
\end{tabular}
\label{trainepoch3}
\end{center}
\end{table}


==> Tables/trainp.tex <==
\begin{table}[H]
\caption{Number of trainable parameters}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & 14190266 & 14223034 & 14190266 & 14149306 & 14182074 & 14149306 \\ \hline
Conv2D & 23026020 & 23029860 & 23026020 & 12492388 & 12498020 & 12492388 \\ \hline
Conv2D t & 1446402 & 1447362 & 1446402 & 775234 & 776642 & 775234 \\ \hline
Conv3D & 7039682 & 7040642 & 7039682 & 3727874 & 3729282 & 3727874 \\ \hline
Conv2.5D & 2676574 & 2680420 & 2676574 & 1434192 & 1437173 & 1434192 \\ \hline
Conv2.5Db & 1604834 & 1607718 & 1604834 & 839506 & 842004 & 839506 \\ \hline
FC t Boundary & 256240 & 260336 & 256240 & 251120 & 255216 & 251120 \\ \hline
Conv1D Boundary & 6908260 & 6912100 & 6908260 & 3617380 & 3623012 & 3617380 \\ \hline
Conv1D t Boundary & 435458 & 436418 & 435458 & \textbf{226114} & 227522 & 226114 \\ \hline
Conv2D Boundary & 2134210 & 2135170 & 2134210 & 1100546 & 1101954 & 1100546 \\ \hline
Conv1.5D Boundary & 1166876 & 1168798 & 1166876 & 604591 & 606544 & 604591 \\ \hline
\end{tabular}
\label{trainp}
\end{center}
\end{table}


==> Tables/trainp2.tex <==
\begin{table}[H]
\caption{Number of trainable parameters}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textbf{0} & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv2D & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv2D t & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv3D & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv2.5D & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv2.5Db & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
FC t Boundary & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv1D Boundary & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv1D t Boundary & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv2D Boundary & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
Conv1.5D Boundary & 0 & 0 & 0 & 0 & 0 & 0 \\ \hline
\end{tabular}
\label{trainp2}
\end{center}
\end{table}


==> Tables/trainuf3.tex <==
\begin{table}[H]
\caption{Train error on full displacement}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{37.57} & \textcolor{red}{21.63} & \textcolor{red}{38.88} & \textcolor{red}{36.75} & \textcolor{red}{13.02} & \textcolor{red}{36.71} \\ \hline
Conv2D & \textcolor{blue}{1.88} & \textcolor{blue}{1.71} & \textcolor{blue}{1.76} & \textcolor{blue}{1.73} & \textcolor{red}{4.62} & \textcolor{blue}{1.76} \\ \hline
Conv2D t & \textcolor{red}{4.36} & \textcolor{red}{4.29} & \textcolor{red}{4.94} & \textcolor{red}{5.81} & \textcolor{red}{4.46} & \textcolor{red}{5.88} \\ \hline
Conv3D & \textcolor{red}{4.07} & \textcolor{blue}{1.11} & \textcolor{blue}{1.31} & \textcolor{blue}{1.60} & \textbf{1.09} & \textcolor{blue}{1.57} \\ \hline
Conv2.5D & \textcolor{blue}{1.72} & \textcolor{blue}{1.50} & \textcolor{blue}{1.69} & \textcolor{blue}{1.83} & \textcolor{blue}{1.37} & \textcolor{blue}{1.72} \\ \hline
Conv2.5Db & \textcolor{red}{4.24} & \textcolor{red}{2.86} & \textcolor{red}{2.96} & \textcolor{red}{2.44} & \textcolor{red}{2.30} & \textcolor{blue}{1.97} \\ \hline
\end{tabular}
\label{TrainUF3}
\end{center}
\end{table}


==> Tables/trainufz3.tex <==
\begin{table}[H]
\caption{Train error on displacement after zoom}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{29.61} & \textcolor{red}{11.52} & \textcolor{red}{32.84} & \textcolor{red}{23.34} & \textcolor{red}{8.42} & \textcolor{red}{25.88} \\ \hline
Conv2D & \textcolor{red}{0.32} & \textcolor{red}{0.21} & \textcolor{red}{0.41} & \textcolor{red}{0.26} & \textcolor{red}{0.31} & \textcolor{red}{0.26} \\ \hline
Conv2D t & \textcolor{red}{2.35} & \textcolor{red}{1.97} & \textcolor{red}{2.21} & \textcolor{red}{2.71} & \textcolor{red}{1.93} & \textcolor{red}{2.75} \\ \hline
Conv3D & \textcolor{red}{1.14} & \textcolor{red}{0.29} & \textcolor{red}{0.33} & \textcolor{red}{0.35} & \textcolor{red}{0.30} & \textcolor{red}{0.44} \\ \hline
Conv2.5D & \textcolor{red}{0.61} & \textcolor{red}{0.58} & \textcolor{red}{0.59} & \textcolor{red}{0.57} & \textcolor{red}{0.46} & \textcolor{red}{0.45} \\ \hline
Conv2.5Db & \textcolor{red}{0.85} & \textcolor{red}{0.78} & \textcolor{red}{0.82} & \textcolor{red}{0.72} & \textcolor{red}{1.01} & \textcolor{red}{0.72} \\ \hline
FC t Boundary & \textcolor{red}{27.66} & \textcolor{red}{9.58} & \textcolor{red}{22.90} & \textcolor{red}{27.24} & \textcolor{red}{9.90} & \textcolor{red}{19.77} \\ \hline
Conv1D Boundary & \textcolor{blue}{0.12} & \textbf{0.08} & \textcolor{blue}{0.11} & \textcolor{blue}{0.15} & \textcolor{blue}{0.10} & \textcolor{blue}{0.10} \\ \hline
Conv1D t Boundary & \textcolor{red}{1.27} & \textcolor{red}{1.20} & \textcolor{red}{1.15} & \textcolor{red}{1.97} & \textcolor{red}{2.01} & \textcolor{red}{1.54} \\ \hline
Conv2D Boundary & \textcolor{red}{0.22} & \textcolor{red}{0.19} & \textcolor{red}{0.24} & \textcolor{red}{0.25} & \textcolor{red}{0.19} & \textcolor{red}{0.22} \\ \hline
Conv1.5D Boundary & \textcolor{red}{0.34} & \textcolor{red}{0.32} & \textcolor{red}{0.25} & \textcolor{red}{0.25} & \textcolor{red}{0.30} & \textcolor{red}{0.26} \\ \hline
\end{tabular}
\label{TrainUFZ3}
\end{center}
\end{table}


==> Tables/trainvf3.tex <==
\begin{table}[H]
\caption{Train error on full velocity}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{9.75} & \textcolor{red}{3.32} & \textcolor{red}{8.43} & \textcolor{red}{8.58} & \textcolor{red}{4.29} & \textcolor{red}{7.76} \\ \hline
Conv2D & \textcolor{red}{2.89} & \textcolor{red}{2.96} & \textcolor{red}{3.66} & \textcolor{red}{2.80} & \textcolor{red}{4.44} & \textcolor{red}{3.03} \\ \hline
Conv2D t & \textcolor{blue}{1.18} & \textbf{1.06} & \textcolor{blue}{1.22} & \textcolor{blue}{1.44} & \textcolor{blue}{1.18} & \textcolor{blue}{1.50} \\ \hline
Conv3D & \textcolor{red}{148.38} & \textcolor{red}{2.45} & \textcolor{red}{2.59} & \textcolor{red}{2.86} & \textcolor{red}{2.56} & \textcolor{red}{2.83} \\ \hline
Conv2.5D & \textcolor{red}{2.96} & \textcolor{red}{2.65} & \textcolor{red}{2.75} & \textcolor{red}{2.73} & \textcolor{red}{2.61} & \textcolor{red}{2.78} \\ \hline
Conv2.5Db & \textcolor{red}{3.14} & \textcolor{red}{2.97} & \textcolor{red}{3.38} & \textcolor{red}{3.15} & \textcolor{red}{2.88} & \textcolor{red}{2.85} \\ \hline
\end{tabular}
\label{TrainVF3}
\end{center}
\end{table}


==> Tables/trainvfz3.tex <==
\begin{table}[H]
\caption{Train error on velocity after zoom}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
& Basic & BN & E & SL & BN \& SL & E \& SL \\ \hline
FC t & \textcolor{red}{17.62} & \textcolor{red}{6.93} & \textcolor{red}{18.39} & \textcolor{red}{13.90} & \textcolor{red}{6.00} & \textcolor{red}{14.49} \\ \hline
Conv2D & \textcolor{red}{0.31} & \textcolor{red}{0.23} & \textcolor{red}{0.36} & \textcolor{red}{0.29} & \textcolor{red}{0.30} & \textcolor{red}{0.28} \\ \hline
Conv2D t & \textcolor{red}{1.44} & \textcolor{red}{1.12} & \textcolor{red}{1.30} & \textcolor{red}{1.60} & \textcolor{red}{1.32} & \textcolor{red}{1.73} \\ \hline
Conv3D & \textcolor{red}{1.23} & \textcolor{red}{0.27} & \textcolor{red}{0.28} & \textcolor{red}{0.30} & \textcolor{red}{0.26} & \textcolor{red}{0.33} \\ \hline
Conv2.5D & \textcolor{red}{0.54} & \textcolor{red}{0.44} & \textcolor{red}{0.47} & \textcolor{red}{0.44} & \textcolor{red}{0.35} & \textcolor{red}{0.41} \\ \hline
Conv2.5Db & \textcolor{red}{0.61} & \textcolor{red}{0.60} & \textcolor{red}{0.64} & \textcolor{red}{0.60} & \textcolor{red}{0.63} & \textcolor{red}{0.55} \\ \hline
FC t Boundary & \textcolor{red}{13.19} & \textcolor{red}{5.81} & \textcolor{red}{13.05} & \textcolor{red}{12.94} & \textcolor{red}{5.86} & \textcolor{red}{10.50} \\ \hline
Conv1D Boundary & \textcolor{blue}{0.15} & \textbf{0.10} & \textcolor{blue}{0.13} & \textcolor{blue}{0.16} & \textcolor{blue}{0.13} & \textcolor{blue}{0.13} \\ \hline
Conv1D t Boundary & \textcolor{red}{0.85} & \textcolor{red}{0.83} & \textcolor{red}{0.77} & \textcolor{red}{1.03} & \textcolor{red}{1.27} & \textcolor{red}{0.94} \\ \hline
Conv2D Boundary & \textcolor{blue}{0.20} & \textcolor{blue}{0.18} & \textcolor{blue}{0.20} & \textcolor{blue}{0.21} & \textcolor{blue}{0.17} & \textcolor{blue}{0.19} \\ \hline
Conv1.5D Boundary & \textcolor{red}{0.24} & \textcolor{red}{0.25} & \textcolor{blue}{0.20} & \textcolor{red}{0.22} & \textcolor{red}{0.23} & \textcolor{red}{0.23} \\ \hline
\end{tabular}
\label{TrainVFZ3}
\end{center}
\end{table}

